On the Statistical Benefits of Curriculum Learning

Curriculum learning (CL) is a commonly used machine learning training strategy. However, we still lack a clear theoretical understanding of CL's benefits. In this paper, we study the benefits of CL in the multitask linear regression problem under both structured and unstructured settings. For both settings, we derive the minimax rates for CL with the oracle that provides the optimal curriculum and without the oracle, where the agent has to adaptively learn a good curriculum. Our results reveal that adaptive learning can be fundamentally harder than the oracle learning in the unstructured setting, but it merely introduces a small extra term in the structured setting. To connect theory with practice, we provide justification for a popular empirical method that selects tasks with highest local prediction gain by comparing its guarantees with the minimax rates mentioned above.

==> Optimal%20Curriculum%20Design%20(Version%209049)/might_be_useful.tex <==

\subsection{Lower bound construction}
To prove the lower bound, we first introduce our lower bound construction.
We construct $2N$ pairs of $(W_S^{(i)}, W_T^{(i)})$, $i = 1, \dots, N$. The first $1, \dots, N$ pairs satisfy:
\begin{enumerate}
    \item $W_T^{(i)}$'s are $2\delta$-separated by the transfer distance;
    \item Let $\mathcal{W}_S$ be a coverage of $\{W_T^{(i)}\}_{i = 1}^{N}$ with error $\Delta$ and $W_S^{(i)} = \argmin_{W \in \mathcal{W}_S} \rho(W, W_T^{(i)})$.
\end{enumerate}

We consider the following $N$-array hypothesis testing problem:
\begin{enumerate}
    \item $J$ is the uniform distribution over the index set $[N] = \{1, 2, \dots, N\}$
    \item Given $J = j$, generate $n_S$, i.i.d samples from $\PP_{W_S^{(i)}}$ and $n_T$ i.i.d. samples from $\PP_{W_T^{(i)}}$.
\end{enumerate}

The goal is to find the true index using the $n_S + n_T$ samples by a testing function $\psi$ from the samples to the indices. We denote the random samples by $Z_{\PP_{S}}$ and $Z_{\PP_{T}}$.

Let $$\psi\left(Z_{\mathbb{P}}, Z_{\mathbb{Q}}\right):=\underset{n \in[N]}{\argmin\ } \rho(\hat{{W}}_{T}, {W}_{T}^{n}).$$

By Fano's inequality, we have 
\begin{align*}
    R_T 
    &\geq \delta^2 \frac{1}{N} \sum_{i = 1}^N \PP\left\{\psi(Z_{\PP_S}, Z_{\PP_T}) \neq i\right\}\\
    &\geq \delta^2 \left(1-\frac{I(J;Z_{\PP_S}) + I(J; Z_{\PP_T}) + \log(2)}{\log(N)} \right)\\
    &\geq \delta^2 \left(1-\frac{n_S I(J;E) + n_T I(J; F) + \log(2)}{\log(N)} \right) \numberthis\label{equ:step1}
\end{align*}

We can bound the mutual information by the following KL-divergence:
\begin{align*}
    I(J; E) \leq \frac{1}{N^2} \sum_{i, j} D_{KL}(\PP_{W_S^{(i)}} \| \PP_{W_S^{(j)}})\\
    I(J; F) \leq \frac{1}{N^2} \sum_{i, j} D_{KL}(\PP_{W_T^{(i)}} \| \PP_{W_T^{(j)}}).
\end{align*}
By calculations, 
$$
    D_{KL}(\PP_{W_S^{(i)}} \| \PP_{W_S^{(j)}}) = \frac{\|\Sigma_S^{1/2}(W_S^{(i)} - W_S^{(j)})\|_{F}^2}{2\sigma_S^2}
$$
$$
    D_{KL}(\PP_{W_T^{(i)}} \| \PP_{W_T^{(j)}}) = \frac{\|\Sigma_T^{1/2}(W_T^{(i)} - W_T^{(j)})\|_{F}^2}{2\sigma_T^2}.
$$

Now consider the following set
$$
    \left\{\eta: \eta={\Sigma}_{T}^{\frac{1}{2}} {W}_{T}^{T} \text{ for some } {W}_{T} \in \mathbb{R}^{k \times d} \|\eta\|_{F} \leq 4 \Delta\right\}.
$$
Let $\{\eta_1, \dots, \eta_N\}$ be a $2\delta$-packing of this set in the $F$-norm. We can find such a packing with $\log(N) \geq rk\log(2\Delta/\delta)$ elements. Number of elements in $\mathcal{W}_S$ is $rk\log(2)$, which we denote by $M$.

We denote the any $j$ by $(g(j), h(j))$, where $m$ is the corresponding index for $\mathcal{W}_S$ and $m_j$ is the index for $j$'s corresponding to the same element. \ziping{We have to assume $\Sigma_S = \Sigma_T$.}

So we get 
\begin{equation}
    D_{KL}(\PP_{W_S^{(j)}}, \PP_{W_S^{(i)}}) \leq \left \{
    \begin{aligned}
        & 0 & \text{ if } g(j) = g(i)\\
        &\frac{32\Delta^2}{\sigma_S^2} &\text{ otherwise}\\
    \end{aligned}
    \right.
\end{equation}
\begin{equation}
    D_{KL}(\PP_{W_T^{(j)}}, \PP_{W_T^{(i)}}) \leq \left \{
    \begin{aligned}
        & \frac{32\delta^2}{\sigma_T^2} & \text{ if } g(j) = g(i)\\
        &\frac{32\Delta^2}{\sigma_T^2} &\text{ otherwise}\\
    \end{aligned}
    \right.
\end{equation}
    
Then we have 
$$
    I(J;E) = \frac{32\Delta^2}{\sigma_S^2} (1 - \frac{1}{M}) \text{ and } I(J;F) = \frac{32\Delta^2}{\sigma_T^2} (1 - \frac{1}{M}) + \frac{1}{M} \frac{32\delta^2}{\sigma_T^2}.
$$

Finally, we have the 
\begin{align*}
    (\ref{equ:step1}) \geq \delta^2 \left(1 - \frac{n_S \frac{32\Delta^2}{\sigma_S^2} (1 - \frac{1}{M}) + n_T \frac{32\Delta^2}{\sigma_T^2} (1 - \frac{1}{M}) + \frac{1}{M} \frac{32\delta^2}{\sigma_T^2} + \log(2)}{\log(N)} \right)
\end{align*}

==> might_be_useful.tex <==

\subsection{Lower bound construction}
To prove the lower bound, we first introduce our lower bound construction.
We construct $2N$ pairs of $(W_S^{(i)}, W_T^{(i)})$, $i = 1, \dots, N$. The first $1, \dots, N$ pairs satisfy:
\begin{enumerate}
    \item $W_T^{(i)}$'s are $2\delta$-separated by the transfer distance;
    \item Let $\mathcal{W}_S$ be a coverage of $\{W_T^{(i)}\}_{i = 1}^{N}$ with error $\Delta$ and $W_S^{(i)} = \argmin_{W \in \mathcal{W}_S} \rho(W, W_T^{(i)})$.
\end{enumerate}

We consider the following $N$-array hypothesis testing problem:
\begin{enumerate}
    \item $J$ is the uniform distribution over the index set $[N] = \{1, 2, \dots, N\}$
    \item Given $J = j$, generate $n_S$, i.i.d samples from $\PP_{W_S^{(i)}}$ and $n_T$ i.i.d. samples from $\PP_{W_T^{(i)}}$.
\end{enumerate}

The goal is to find the true index using the $n_S + n_T$ samples by a testing function $\psi$ from the samples to the indices. We denote the random samples by $Z_{\PP_{S}}$ and $Z_{\PP_{T}}$.

Let $$\psi\left(Z_{\mathbb{P}}, Z_{\mathbb{Q}}\right):=\underset{n \in[N]}{\argmin\ } \rho(\hat{{W}}_{T}, {W}_{T}^{n}).$$

By Fano's inequality, we have 
\begin{align*}
    R_T 
    &\geq \delta^2 \frac{1}{N} \sum_{i = 1}^N \PP\left\{\psi(Z_{\PP_S}, Z_{\PP_T}) \neq i\right\}\\
    &\geq \delta^2 \left(1-\frac{I(J;Z_{\PP_S}) + I(J; Z_{\PP_T}) + \log(2)}{\log(N)} \right)\\
    &\geq \delta^2 \left(1-\frac{n_S I(J;E) + n_T I(J; F) + \log(2)}{\log(N)} \right) \numberthis\label{equ:step1}
\end{align*}

We can bound the mutual information by the following KL-divergence:
\begin{align*}
    I(J; E) \leq \frac{1}{N^2} \sum_{i, j} D_{KL}(\PP_{W_S^{(i)}} \| \PP_{W_S^{(j)}})\\
    I(J; F) \leq \frac{1}{N^2} \sum_{i, j} D_{KL}(\PP_{W_T^{(i)}} \| \PP_{W_T^{(j)}}).
\end{align*}
By calculations, 
$$
    D_{KL}(\PP_{W_S^{(i)}} \| \PP_{W_S^{(j)}}) = \frac{\|\Sigma_S^{1/2}(W_S^{(i)} - W_S^{(j)})\|_{F}^2}{2\sigma_S^2}
$$
$$
    D_{KL}(\PP_{W_T^{(i)}} \| \PP_{W_T^{(j)}}) = \frac{\|\Sigma_T^{1/2}(W_T^{(i)} - W_T^{(j)})\|_{F}^2}{2\sigma_T^2}.
$$

Now consider the following set
$$
    \left\{\eta: \eta={\Sigma}_{T}^{\frac{1}{2}} {W}_{T}^{T} \text{ for some } {W}_{T} \in \mathbb{R}^{k \times d} \|\eta\|_{F} \leq 4 \Delta\right\}.
$$
Let $\{\eta_1, \dots, \eta_N\}$ be a $2\delta$-packing of this set in the $F$-norm. We can find such a packing with $\log(N) \geq rk\log(2\Delta/\delta)$ elements. Number of elements in $\mathcal{W}_S$ is $rk\log(2)$, which we denote by $M$.

We denote the any $j$ by $(g(j), h(j))$, where $m$ is the corresponding index for $\mathcal{W}_S$ and $m_j$ is the index for $j$'s corresponding to the same element. \ziping{We have to assume $\Sigma_S = \Sigma_T$.}

So we get 
\begin{equation}
    D_{KL}(\PP_{W_S^{(j)}}, \PP_{W_S^{(i)}}) \leq \left \{
    \begin{aligned}
        & 0 & \text{ if } g(j) = g(i)\\
        &\frac{32\Delta^2}{\sigma_S^2} &\text{ otherwise}\\
    \end{aligned}
    \right.
\end{equation}
\begin{equation}
    D_{KL}(\PP_{W_T^{(j)}}, \PP_{W_T^{(i)}}) \leq \left \{
    \begin{aligned}
        & \frac{32\delta^2}{\sigma_T^2} & \text{ if } g(j) = g(i)\\
        &\frac{32\Delta^2}{\sigma_T^2} &\text{ otherwise}\\
    \end{aligned}
    \right.
\end{equation}
    
Then we have 
$$
    I(J;E) = \frac{32\Delta^2}{\sigma_S^2} (1 - \frac{1}{M}) \text{ and } I(J;F) = \frac{32\Delta^2}{\sigma_T^2} (1 - \frac{1}{M}) + \frac{1}{M} \frac{32\delta^2}{\sigma_T^2}.
$$

Finally, we have the 
\begin{align*}
    (\ref{equ:step1}) \geq \delta^2 \left(1 - \frac{n_S \frac{32\Delta^2}{\sigma_S^2} (1 - \frac{1}{M}) + n_T \frac{32\Delta^2}{\sigma_T^2} (1 - \frac{1}{M}) + \frac{1}{M} \frac{32\delta^2}{\sigma_T^2} + \log(2)}{\log(N)} \right)
\end{align*}
